The distribution amplitude of the $\eta_c$-meson at leading twist from Lattice QCD

Distribution amplitudes are functions of non-perturbative matrix elements describing the hadronization of quarks and gluons. Thanks to factorization theorems, they can be used to compute the scattering amplitude of high-energy processes. Recently, new ideas have allowed their computation using lattice QCD, which should provide us with a general, fully relativistic determination. We present the first lattice calculation of the $\eta_c$-meson distribution amplitude at leading twist. Starting from the relevant matrix element in discrete Euclidean space on a set of $N_f=2$ CLS ensembles, we explain the method to connect to continuum Minkowski spacetime. After addressing several sources of systematic uncertainty, we compare to Dyson-Schwinger and non-relativistic QCD determinations of this quantity. We find significant deviations between the latter and our result even at small Ioffe times.

==> tables/time-spread-covariance.tex <==
\begin{tabular}{ccccccc}
\toprule
          & $\lambda$  & $a_{1,2}$ & $b_{1,2}$ & $c_{1,2}$ & $e_{1,2}$ & $d_{1,2}$ \\
\midrule
$\lambda$ &  0.015141 & -0.001664 &  0.009456 &  0.000276 & -0.000188 &  0.001106 \\
$a_{1,2}$ & -0.001664 &  0.326381 & -0.000390 &  0.000167 &  0.088220 &  0.008977 \\
$b_{1,2}$ &  0.009456 & -0.000390 &  0.006154 &  0.000145 &  0.000080 &  0.001114 \\
$c_{1,2}$ &  0.000276 &  0.000167 &  0.000145 &  0.000023 &  0.000047 &  0.000034 \\
$d_{1,2}$ & -0.000188 &  0.088220 &  0.000080 &  0.000047 &  0.023856 &  0.002551 \\
$e_{1,2}$ &  0.001106 &  0.008977 &  0.001114 &  0.000034 &  0.002551 &  0.003371 \\
\midrule
Mean &  2.730 & -7.576 &  0.883 & -0.042 & -2.218 & -0.080 \\
\bottomrule
\end{tabular}
